Balanced Gradient Sample Retrieval for Enhanced Knowledge Retention in Proxy-based Continual Learning

Continual learning in deep neural networks often suffers from catastrophic forgetting, where representations for previous tasks are overwritten during subsequent training. We propose a novel sample retrieval strategy from the memory buffer that leverages both gradient-conflicting and gradient-aligned samples to effectively retain knowledge about past tasks within a supervised contrastive learning framework. Gradient-conflicting samples are selected for their potential to reduce interference by re-aligning gradients, thereby preserving past task knowledge. Meanwhile, gradient-aligned samples are incorporated to reinforce stable, shared representations across tasks. By balancing gradient correction from conflicting samples with alignment reinforcement from aligned ones, our approach increases the diversity among retrieved instances and achieves superior alignment in parameter space, significantly enhancing knowledge retention and mitigating proxy drift. Empirical results demonstrate that using both sample types outperforms methods relying solely on one sample type or random retrieval. Experiments on popular continual learning benchmarks in computer vision validate our method's state-of-the-art performance in mitigating forgetting while maintaining competitive accuracy on new tasks.

==> sec/3_methodology.tex <==
\section{Methodology}\label{Method}
\label{Method}
In this section, we introduce our approach to improving continual learning performance by strategically selecting positive and negative loss change samples within a contrastive learning framework that utilizes prototypes. We first formulate the continual learning problem under experience replay, outline our sample selection strategy, and provide a theoretical analysis demonstrating the superiority of our method in mitigating catastrophic forgetting and promoting effective task learning.


\subsection{Contrastive Learning with Prototypes}

In our method, we integrate prototype-based representations with contrastive learning to maximize inter-class separation and intra-class cohesion, enhancing the discriminative power of embeddings. Let $\Phi$ be the model parameters, $h(x; \Phi)$ be the embedding of input $x$, and $w_y$ be the prototype for class $y$. The training objective encourages $h(x; \Phi)$ to align with its corresponding prototype $w_y$ while diverging from other class prototypes.

The prototype-based contrastive loss is defined as:
\begin{equation}
L_{\text{ctr.}} = \mathbb{E}_{(x, y) \sim \mathcal{D}} \left[ -\log \left( \frac{\exp\left( \gamma \langle h(x; \Phi), w_y \rangle \right)}{\sum_{j \in C_B} \exp\left( \gamma \langle h(x; \Phi), w_j \rangle \right)} \right) \right],
\label{eq:contrastive_loss}
\end{equation}
where $\gamma$ is a scaling factor, $\langle \cdot, \cdot \rangle$ denotes the cosine similarity, and $C_B$ is the set of class indices in the current training batch.

\subsection{Continual Learning with Experience Replay}\label{PF}
Continual learning aims to enable a model to sequentially learn tasks $\{ \mathcal{T}_1, \mathcal{T}_2, \dots, \mathcal{T}_T \}$, where data from past tasks are generally unavailable during training on the current task $\mathcal{T}_t$. The primary challenge lies in learning new tasks without forgetting previously learned knowledge.

Experience replay addresses this issue by maintaining a memory buffer $\mathcal{M}$ that stores a subset of samples from past tasks. During training on the current task, the model updates its parameters using both current task data $\mathcal{D}_t$ and memory samples $\mathcal{M}$, ensuring past task information is preserved.


\subsubsection{MIR method}
MIR method is ... . 

\subsection{Proposed Sample Selection Strategy}

To further enhance performance, we propose a sample selection strategy that combines both positive and negative loss change samples from the memory buffer. This strategy aims to balance the contributions of the gradient during training, taking advantage of the complementary benefits of both types of samples.

\subsubsection{Gradient alignment of selected samples and samples from the batch}
We denote a cross-entropy loss for sample $x$ as $l_\Phi(x)$, and $L_\Phi(X_t)$ to be loss over the batch of samples $X_t = \{x_i\}$ 
\begin{equation}
    L_\Phi(X_t) = \frac{1}{\#X_t} \sum_{i=1}^{\#X_t} l_\Phi(x_i)
\end{equation}
We define criterion $f$:
\begin{equation}
    f(x) = l_{\Phi'}(x) - l_\Phi(x),
\end{equation}
and choose $k$ highest and lowest values. The highest are motivated in MIR. However, taking the lowest values also makes sense, because ... . We expand sample loss into first order Taylor series:
\begin{equation}
    l_{\Phi'}(x)  \approx l_\Phi(x) + (\Phi' - \Phi)^\top \nabla_{\Phi} l_\Phi(x).
\end{equation}
Since
\begin{equation}
\Phi' = \Phi - \alpha \nabla_\Phi L_\Phi (X_t),
\end{equation}
we can approximate $f$ by:
\begin{equation}
    f(x) \approx  - \alpha (\nabla_\Phi L_\Phi (X_t))^\top \nabla_{\Phi} l_\Phi(x)
\end{equation}
MIR likes it when the gradients are aligned $((\nabla_\Phi L_\Phi (X_t))^\top \nabla_{\Phi} l_\Phi(x)) > 0$, and the alignment is very weak, or when gradients are NOT aligned, and the misalignment is very strong.
\\
\\
IMIR likes it when the gradients are NOT aligned $((\nabla_\Phi L_\Phi (X_t))^\top \nabla_{\Phi} l_\Phi(x)) < 0$, and the misalignment is very weak, or when gradients are aligned, and the alignment is very strong.
\\
\\
So we include samples from IMIR to increase gradient alignment 

\subsection{Prototypes drift}
% % ======================================================================
% % ======================================================================
% % OLD VERSION STARTS HERE
% % ======================================================================
% % ======================================================================
% \subsubsection{Computation of Loss Change}
% Following the methodology outlined in \cite{aljundi2019online}, we compute the loss change to evaluate the impact of each memory sample on the current model. This approach involves simulating an additional gradient step, which aids in identifying the most interfered samples, thereby enhancing rehearsal effectiveness and mitigating catastrophic forgetting. Specifically, after training on the current task $\mathcal{T}_t$, the loss change $\Delta L_x$ for each memory sample $x \in \mathcal{M}$ is computed as:

% \begin{equation}
% \Delta L_x = L_{\text{ctr.}}(x; \Phi_{\text{old}}) - L_{\text{ctr.}}(x; \Phi_{\text{new}}),
% \end{equation}

% where $\Phi_{\text{old}}$ and $\Phi_{\text{new}}$ denote the model parameters before and after training on $\mathcal{T}_t$, respectively. Based on $\Delta L_x$, we select:

% \begin{itemize}
%     \item \textbf{Positive Loss Change Samples ($S_{+}$)}: The top $C$ samples with the largest positive loss change ($\Delta L_x > 0$).
%     \item \textbf{Negative Loss Change Samples ($S_{-}$)}: The top $C$ samples with the largest negative loss change ($\Delta L_x < 0$).
% \end{itemize}

% \subsubsection{Gradient Formulation and Analysis}

% Let $G_{\text{cur}}$ denote the gradient of the loss on the current task $\mathcal{D}_t$, and $G_{\text{mem}}$ denote the gradient contribution from memory samples. The total gradient is expressed as:

% \begin{equation}
% G_{\text{total}} = G_{\text{cur}} + \gamma G_{\text{mem}},
% \end{equation}

% where

% \begin{equation}
% G_{\text{mem}} = \alpha_+ G_{S_{+}} + \alpha_- G_{S_{-}},
% \end{equation}

% with $\alpha_+ = \frac{|S_{+}|}{|S|}$ and $\alpha_- = \frac{|S_{-}|}{|S|}$ representing the proportions of positive and negative loss change samples, respectively. For the combined strategy, we assume $|S_{+}| = |S_{-}| = C$, resulting in $\alpha_+ = \alpha_- = 0.5$. In contrast, single-type strategies utilize $2C$ samples of one type, leading to $\alpha_+ = 1$ or $\alpha_- = 1$.

% \paragraph{Gradient Interactions}

% The interactions between the current gradient and memory gradients are characterized by:

% \begin{align}
% G_{\text{cur}}^\top G_{S_{+}} &= \|G_{\text{cur}}\| \|G_{S_{+}}\| \cos \theta_{+}, \quad \text{with} \ \cos \theta_{+} < 0, \\
% G_{\text{cur}}^\top G_{S_{-}} &= \|G_{\text{cur}}\| \|G_{S_{-}}\| \cos \theta_{-}, \quad \text{with} \ \cos \theta_{-} > 0.
% \end{align}
% % ===============================================
% \subsubsection{Comparison of Combined Strategy with Positive-Only and Negative-Only Strategies}

% We compare the expected loss reductions of the combined strategy ($S$) with the positive-only ($S_{+}^{2C}$) and negative-only ($S_{-}^{2C}$) strategies to show that the combined strategy results in a greater loss reduction.

% \paragraph{Loss Reduction Differences}

% We define the differences in expected loss reductions as:

% \begin{align}
% \Delta L_{\text{neg-only}} - \Delta L_{\text{comb.}} &= \eta \left( \| G_{\text{total}}^{\text{comb}} \|^2 - \| G_{\text{total}}^{\text{neg-only}} \|^2 \right), \label{eq:delta_neg_comb} \\
% \Delta L_{\text{pos-only}} - \Delta L_{\text{comb.}} &= \eta \left( \| G_{\text{total}}^{\text{comb}} \|^2 - \| G_{\text{total}}^{\text{pos-only}} \|^2 \right). \label{eq:delta_pos_comb}
% \end{align}
% \vspace{-0.5mm}
% Here, $G_{\text{total}}^{\text{comb}}$ represents the combined strategy gradient, defined as $G_{\text{cur}} + \gamma (\alpha_+ G_{S_{+}} + \alpha_- G_{S_{-}})$, where $\alpha_+ = \alpha_- = 0.5$. The negative-only strategy gradient is $G_{\text{total}}^{\text{neg-only}} = G_{\text{cur}} + \gamma G_{S_{-}^{2C}}$, and the positive-only strategy gradient is $G_{\text{total}}^{\text{pos-only}} = G_{\text{cur}} + \gamma G_{S_{+}^{2C}}$. Additionally, we assume that $G_{S_{-}^{2C}} = 2G_{S_{-}}$ and $G_{S_{+}^{2C}} = 2G_{S_{+}}$.


% \subsubsection{Gradient Norms}

% The gradient norms for each strategy can be expressed as follows. For the combined strategy, we have:
% \vspace{-2mm}
% \begin{align}
% \| G_{\text{total}}^{\text{comb}} \|^2 &= \| G_{\text{cur}} \|^2 + \gamma G_{\text{cur}}^\top (G_{S_{+}} + G_{S_{-}}) \nonumber \\
% &\quad + \gamma^2 \left( \frac{1}{4} \| G_{S_{+}} \|^2 + \frac{1}{2} G_{S_{+}}^\top G_{S_{-}} + \frac{1}{4} \| G_{S_{-}} \|^2 \right). \label{eq:combined_norm}
% \end{align}
% For the negative-only gradient norm is given by:
% \begin{equation}
% \| G_{\text{total}}^{\text{neg-only}} \|^2 = \| G_{\text{cur}} \|^2 + 2 \gamma G_{\text{cur}}^\top G_{S_{-}} + 4 \gamma^2 \| G_{S_{-}} \|^2. \label{eq:neg_only_norm}
% \end{equation}
% Similarly, for the positive-only gradient norm is:
% \begin{equation}
% \| G_{\text{total}}^{\text{pos-only}} \|^2 = \| G_{\text{cur}} \|^2 + 2 \gamma G_{\text{cur}}^\top G_{S_{+}} + 4 \gamma^2 \| G_{S_{+}} \|^2. \label{eq:pos_only_norm}
% \end{equation}

% \subsubsection{Analysis of Differences}

% To compare the combined strategy with the negative-only strategy, we evaluate the difference:
% \vspace{-2mm}
% \begin{align}
% \Delta_{\text{neg}} &= \| G_{\text{total}}^{\text{comb}} \|^2 - \| G_{\text{total}}^{\text{neg-only}} \|^2 \nonumber \\
% &= \gamma (G_{\text{cur}}^\top G_{S_{+}} - G_{\text{cur}}^\top G_{S_{-}}) \nonumber \\
% &\quad + \gamma^2 \left( \frac{1}{4} \| G_{S_{+}} \|^2 + \frac{1}{2} G_{S_{+}}^\top G_{S_{-}} - \frac{15}{4} \| G_{S_{-}} \|^2 \right). \label{eq:delta_neg}
% \end{align}
% Using typical gradient properties such as $G_{\text{cur}}^\top G_{S_{+}} < 0$, $G_{\text{cur}}^\top G_{S_{-}} > 0$, and $G_{S_{+}}^\top G_{S_{-}} \approx 0$ (Gradients are nearly orthogonal in higher dimensional spaces), we can observe that the term $\gamma (G_{\text{cur}}^\top G_{S_{+}} - G_{\text{cur}}^\top G_{S_{-}})$ is negative, and the $\gamma^2$ terms are dominated by $-\frac{15}{4} \| G_{S_{-}} \|^2$. This results in $\Delta_{\text{neg}} < 0$, implying:
% \begin{equation}
% \Delta L_{\text{comb.}} < \Delta L_{\text{neg-only}}.
% \end{equation}
% Similarly, for the comparison between the combined strategy and the positive-only strategy:
% \begin{align}
% \Delta_{\text{pos}} &= \| G_{\text{total}}^{\text{comb}} \|^2 - \| G_{\text{total}}^{\text{pos-only}} \|^2 \nonumber \\
% &= \gamma (G_{\text{cur}}^\top G_{S_{-}} - G_{\text{cur}}^\top G_{S_{+}}) \nonumber \\
% &\quad + \gamma^2 \left( \frac{1}{4} \| G_{S_{-}} \|^2 + \frac{1}{2} G_{S_{+}}^\top G_{S_{-}} - \frac{15}{4} \| G_{S_{+}} \|^2 \right). \label{eq:delta_pos}
% \end{align}
% \vspace{-3mm}
% Given the same gradient properties, $\Delta_{\text{pos}} < 0$, leading to:
% \begin{equation}
% \Delta L_{\text{comb.}} < \Delta L_{\text{pos-only}}.
% \end{equation}

% \subsubsection{Conclusion}

% The negative values of $\Delta_{\text{neg}}$ and $\Delta_{\text{pos}}$ confirm that:
% \begin{equation}
% \Delta L_{\text{comb.}} < \Delta L_{\text{neg-only}}, \quad \Delta L_{\text{comb.}} < \Delta L_{\text{pos-only}}.
% \end{equation}

% This demonstrates that the combined strategy achieves a greater expected loss reduction than both the positive-only and negative-only strategies.

% % ======================================================================
% % ======================================================================
% % OLD VERSION ENDS HERE
% % ======================================================================
% % ======================================================================


% %Problem formulation
% % Class Incremental Learning (CIL) aims to train models on sequential tasks, each introducing new classes, without forgetting previously learned information. Traditional neural networks suffer from catastrophic forgetting, where learning new classes degrades performance on old ones.

% % The objective in CIL is to balance learning new classes while preserving old knowledge. Let \( f_\theta \) be a neural network with parameters \(\theta\), trained on \( T \) tasks. Each task \( t \) has a dataset \( \mathcal{D}^t = \{(x_i^t, y_i^t)\}_{i=1}^{N_t} \). The task-specific loss \( \mathcal{L}^t(\theta) \) is typically the cross-entropy loss:

% % \[
% % \mathcal{L}^t(\theta) = - \sum_{i=1}^{N_t} \sum_{c=1}^{C_t} y_{ic}^t \log \left( f_\theta(x_i^t) \right)
% % \]

% % where \( C_t \) is the number of classes in task \( t \).

% % In CIL, the challenge is to continually update the model with new tasks while maintaining its performance on previous tasks. This involves designing algorithms that can effectively balance learning new information without degrading the performance on previously learned tasks.

% % In summary, the goal of CIL is to develop models capable of learning new classes incrementally while retaining previously learned knowledge, thus achieving a balance between acquiring new information and preserving old knowledge for lifelong learning.


% Class Incremental Learning (CIL) aims to train models on sequential tasks, each introducing new classes, without forgetting previously learned information. Traditional neural networks suffer from catastrophic forgetting, where learning new classes degrades performance on old ones.

% The objective in CIL is to balance learning new classes while preserving old knowledge. Let \( f_\theta \) be a neural network with parameters \(\theta\), trained on \( T \) tasks. Each task \( t \) has a dataset \( \mathcal{D}^t = \{(x_i^t, y_i^t)\}_{i=1}^{N_t} \). The task-specific loss \( \mathcal{L}^t(\theta) \) is typically the cross-entropy loss:
% \vspace{-2mm}
% \begin{equation}
% \mathcal{L}^t(\theta) = - \sum_{i=1}^{N_t} \sum_{c=1}^{C_t} y_{ic}^t \log \left( f_\theta(x_i^t) \right)
% \end{equation}
% \vspace{-4mm}

% where \( C_t \) is the number of classes in task \( t \).
% To address catastrophic forgetting, a memory buffer \(\mathcal{M}\) is used to store a subset of samples from previous tasks. During training on a new task, samples from the memory buffer are selected and combined with the current task samples to optimize the model. The selection of appropriate samples is crucial for effective learning and minimizing the loss.

% The total loss function for task \( t \), including samples from the memory buffer, can be formulated as:
% \vspace{-1mm}
% \begin{equation}
% \mathcal{L}_{\text{total}}^t(\theta) = \mathcal{L}^t(\theta) + \sum_{(x_i^m, y_i^m) \in \mathcal{M}} \mathcal{L}^m(\theta)
% \end{equation}
% \vspace{-4mm}

% where \(\mathcal{L}^m(\theta)\) represents the loss for samples from the memory buffer. This approach ensures that the model not only focuses on the current task but also reinforces the knowledge from previous tasks.
% % In CIL, the challenge is to continually update the model with new tasks while maintaining its performance on previous tasks. This involves designing algorithms that can effectively balance learning new information without degrading the performance on previously learned tasks.

% % In summary, the goal of CIL is to develop models capable of learning new classes incrementally while retaining previously learned knowledge. By utilizing a memory buffer and selecting appropriate samples from previous tasks, models can achieve a balance between acquiring new information and preserving old knowledge, thus enabling lifelong learning.


% % \begin{wrapfigure}[15]{R}{0.6\textwidth} % Adjusted the number of lines and used 'R' instead of 'r'

% %   \begin{center}
% %   \vspace{-20pt} % 
% %     \includegraphics[width=0.6\textwidth]{figs/sample_hardness.pdf} % Ensured the width matches the wrap width
% %   \end{center}
% %   \vspace{-2mm}
% %   \caption{Hardness measures the likelihood of changes in the level of prediction. We observe a reversal in sample difficulty between Maximal interfered and Minimal interfered as class incremental learning progresses.}
% %   \label{fig:main}
% % \end{wrapfigure}
% % \vspace{-2mm}
% % \subsection{Loss Change and Hardness}\label{LC&H}%Loss Change and Hardness
% % \vspace{-2mm}

% \begin{figure*}[t]
%     \centering
%     \vspace{-20pt} 
%     \includegraphics[width=0.9\textwidth]{figs/sample_hardness.pdf} % 根据需要调整宽度
%     \vspace{-2mm}
%     \caption{Hardness measures the likelihood of changes in the level of prediction. We observe a reversal in sample difficulty between Maximal interfered and Minimal interfered as class incremental learning progresses.}
%     \label{fig:main}
%     \vspace{-2mm} 
% \end{figure*}
% \vspace{-2mm}
% \subsection{Loss Change and Hardness}\label{LC&H} % Loss Change and Hardness
% \vspace{-2mm}
% % Many continual learning methods utilize additional memory to store samples from previous tasks and augment current data with samples from older tasks to prevent catastrophic forgetting. The natural question emerges: which samples from the buffer should be retrieved at the current stage to maximize model performance and minimize forgetting? Aljundi et al. \cite{aljundi2019online}  propose a criterion for selecting samples that are expected to be most negatively impacted by upcoming parameter updates, producing consistent gains over random sampling based on loss change. 

% Many continual learning methods utilize additional memory to store samples from previous tasks, augmenting current data with samples from older tasks to prevent catastrophic forgetting. This raises the question: which samples from the buffer should be retrieved at the current stage to maximize model performance and minimize forgetting? Aljundi et al. \cite{aljundi2019online} propose a criterion for selecting samples that are expected to be most negatively impacted by upcoming parameter updates, yielding consistent gains over random sampling based on loss change.



% % Given a standard objective $\min_{\theta} \mathcal{L}(f_{\theta}(\mathbf{X}_t), \mathbf{Y}_t)$, when receiving sample(s) $\mathbf{X}_t$ the would-be parameters update from the incoming batch are estimated as $\theta^v = \theta - \alpha \nabla \mathcal{L}(f_{\theta}(\mathbf{X}_t), \mathbf{Y}_t)$, with learning rate $\alpha$. The Loss Change criterion is there by defined as: $l(f_{\theta^v}(x), y) - l(f_{\theta}(x), y)$, where $l$ is the loss function. Essentially, selecting samples with increasing loss from the buffer acts as a regularization method to prevent the model from forgetting these samples while learning new ones. However, we occasionally find that adopting the opposite strategy — consistently selecting the samples with the largest negative loss — can achieve results just as competitive as selecting those with the largest positive loss. These results are presented together with \S\ref{ablation}.

% Given a standard objective $\min_{\theta} \mathcal{L}(f_{\theta}(X_n), Y_n)$, when receiving sample(s) $X_n$, the would-be parameter update from the incoming batch is estimated as $\theta^v = \theta - \alpha \nabla \mathcal{L}(f_{\theta}(X_n), Y_n)$, with learning rate $\alpha$. The Loss Change criterion is defined as: $\mathcal{L}(f_{\theta^v}(x_i), y_i) - \mathcal{L}(f_{\theta}(x_i), y_i)$, where $\mathcal{L}$ is the loss function. Essentially, selecting samples with increasing loss from the buffer acts as a regularization method to prevent the model from forgetting these samples while learning new ones. However, we occasionally find that adopting the opposite strategy—consistently selecting samples with the largest negative loss—can achieve results as competitive as selecting those with the largest positive loss. These results are presented in \S\ref{ablation}.


% % \begin{figure*}[h]
% %   \centering
% %       \includegraphics[width=1 \linewidth]{figs/sample_hardness.pdf}
% % \caption{Hardness measures the likelihood of changes in the level of prediction}
% %     \label{fig:main}
% % % \vspace{-6pt}
% % \end{figure*}

% We use a hardness metric slightly different from the definition of hardness presented in~\cite{zhou2020curriculum}, defined as $|f_{\theta^v}(x_i) - f_{\theta}(x_i)|$. This metric offers a more intuitive evaluation of prediction-level variation, enabling us to assess the extent of uncertainty within a sample's prediction.


% Using hardness as an analytical metric, we evaluated the PCR~\cite{lin2023pcr} model across 20 tasks on the CIFAR-100 dataset in a class-incremental learning (CIL) manner (see \S\ref{ES} for more details). Samples were retrieved from the buffer according to three distinct strategies: Maximal Interfered, Minimal Interfered, and Random.

% As shown in Figure \ref{fig:main}, the 20 sub-tasks were each trained for 50 epochs in a CIL manner. We observed a reversal in the hardness magnitude of the samples selected based on maximal interfered and minimal interfered strategies as the training progressed. In the first two tasks, the Minimal Interfered sample shows similar hardness to the random sample, while the Maximal Interfered sample demonstrates greater hardness. However, starting from the fourth task, the hardness of the Minimal Interfered sample surpasses that of the Maximal Interfered sample, and the hardness of the Maximal Interfered sample begins to converge towards the hardness of the random sample.
% %\vspace{-3mm}

% % \begin{figure}[htbp]
% % \vspace{-4mm}
% %     \centering
% %     % Adjust the spacing between the figures
% %     \setlength{\tabcolsep}{-10pt} % Adjust column spacing
% %     \renewcommand{\arraystretch}{-5} % Adjust row spacing

% %     \begin{tabular}{cc}
% %         \begin{adjustbox}{valign=t} % To align the top of the images
% %             \begin{subfigure}[t]{0.5\textwidth} % Adjust width of each subfigure
% %                 \centering
% %                 \includegraphics[width=\textwidth]{figs/Rank_Difference_steps1.pdf}
% %                 % \caption{Subfigure 1}
% %                 % \label{fig:sub1}
% %             \end{subfigure}
% %         \end{adjustbox} &
% %         \begin{adjustbox}{valign=t}
% %             \begin{subfigure}[t]{0.5\textwidth}
% %                 \centering
% %                 \includegraphics[width=\textwidth]{figs/Rank_Difference_steps500.pdf}
% %                 % \caption{Subfigure 2}
% %                 % \label{fig:sub2}
% %             \end{subfigure}
% %         \end{adjustbox} \\ % Start new row
% %         \begin{adjustbox}{valign=t}
% %             \begin{subfigure}[t]{0.5\textwidth}
% %                 \centering
% %                 \includegraphics[width=\textwidth]{figs/Rank_Difference_steps1000.pdf}
% %                 % \caption{Subfigure 3}
% %                 % \label{fig:sub3}
% %             \end{subfigure}
% %         \end{adjustbox} &
% %         \begin{adjustbox}{valign=t}
% %             \begin{subfigure}[t]{0.5\textwidth}
% %                 \centering
% %                 \includegraphics[width=\textwidth]{figs/correlation_over_steps.pdf}
% %                 % \caption{Subfigure 4}
% %                 % \label{fig:sub4}
% %             \end{subfigure}
% %         \end{adjustbox}
% %     \end{tabular}

% %     \caption{Histogram showing the differences in rankings of loss change and hardness (prediction flips) over time. As training progresses (from step 1 to step 1000), more samples display smaller rank differences, indicating an established relationship between loss changes and hardness (prediction flips), though some samples remain difficult to optimize.}
% %     \label{fig:rank}
% %     \vspace{-2mm}
% % \end{figure}
% \begin{figure*}[htbp]
% \vspace{-4mm}
%     \centering
%     \setlength{\tabcolsep}{2pt} 
%     \renewcommand{\arraystretch}{1} 

%     \begin{tabular}{cc}
%         \begin{subfigure}[t]{0.48\textwidth} 
%             \centering
%             \includegraphics[width=\textwidth]{figs/Rank_Difference_steps1.pdf}
%             % \caption{Subfigure 1}
%             % \label{fig:sub1}
%         \end{subfigure} &
%         \begin{subfigure}[t]{0.48\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{figs/Rank_Difference_steps500.pdf}
%             % \caption{Subfigure 2}
%             % \label{fig:sub2}
%         \end{subfigure} \\
%         \begin{subfigure}[t]{0.48\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{figs/Rank_Difference_steps1000.pdf}
%             % \caption{Subfigure 3}
%             % \label{fig:sub3}
%         \end{subfigure} &
%         \begin{subfigure}[t]{0.48\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{figs/correlation_over_steps.pdf}
%             % \caption{Subfigure 4}
%             % \label{fig:sub4}
%         \end{subfigure}
%     \end{tabular}

%     \caption{Histogram showing the differences in rankings of loss change and hardness (prediction flips) over time. As training progresses (from step 1 to step 1000), more samples display smaller rank differences, indicating an established relationship between loss changes and hardness (prediction flips), though some samples remain difficult to optimize.}
%     \label{fig:rank}
%     \vspace{-2mm}
% \end{figure*}

% Additionally, we investigated whether certain samples exhibit a small change in loss while undergoing a significant change in prediction, or conversely, a large change in loss with stable predictions. To explore this, we utilized samples from the test set, considering the model's weights at various time points and the gradients, to compute and rank the changes in loss and hardness (prediction flips). We then visualized a histogram depicting the differences in these rankings, as illustrated in Figure \ref{fig:rank}.

% The histogram reveals that as the model progresses (from step 1 to step 500 and step 1000), an increasing number of samples display smaller rank differences, and the overall distribution becomes progressively long-tailed. This trend suggests that training gradually establishes a relationship between loss changes and hardness (prediction flips), which is also evident from the correlation graph. Despite this, some samples remain difficult to optimize even at the end of training. Hence, it is essential to implement specific strategies to address these challenging samples and minimize ineffective training.




% % Additionally, we also consider another criterion, the prediction flip, which is calculated as $|f_{\theta^v}(x) - f_{\theta}(x)|$. Loss change measures the consistency of the samples with the current direction of the model's optimization whereas prediction flips offer a more intuitive assessment of changes at the prediction level.


% % ############################
% % {\color{red} I would define here two criteria - I started doing it but am unsure if LsC is calculated per batch. CRUCIAL QUESTION: WHAT DO WE LEAVE OUT TAKING INTO CONSIDERATION ONLY LsC? WHY DO WE NEED TO LOOK AT LtC AS WELL?}

% % Loss change: 
% % $$LsC = \sum_B |\mathcal{L} (\text{Softmax}(y^{t-1})) - \mathcal{L} (\text{Softmax}(y^{t}))|$$
% % Logits change: 
% % $$LtC = \sum_B |y^{t-1} - y^{t}|$$
% % {\color{red} This paper argues that MIR is not a sufficient criterion because of hardness. Furthermore, our findings indicate that relaxing the sampling strategy by reducing buffer size enhances the diversity of tail-sampling, which in turn improves model performance.}
% % ############################

% \subsection{Downsizing the buffer}\label{BD}
% \vspace{-2mm}
% In the previous paragraph, we discuss the necessity of sampling from both tails of Loss-Change distribution. In this paragraph, we further argue that sampling "milder" extreme values, i.e., values closer to the mean, leads to improved tail coverage. We achieve this by downsizing the sample size drawn from the buffer. Intuitively, $r$ maximum values from the sample with size $2n$ are, on average, bigger than $r$ maximum values sampled from the sample with size $n$.
% \\
% \\
% More formally, let $U_1, \ldots, U_n$ be an iid random sample with density $f_U$ and cumulative distribution function $F_U$. The distribution of $r$'th order statistic is given by $f_U{_{[r]}}(u) =\frac{n!}{(r-1)!(n-r)!} f_U(u)F_U(u)^{r-1}(1-F_U(u))^{n-r}$. We are interested in the relations between expected values $EU_{[n-r]}$, and partial ranges $EU_{[n]} - EU_{[n-r]}$ between samples with $n$ and $2n$ elements. We can calculate the expectation of $r$'th order statistic as follows: 
% \begin{equation}
%     EU_{[r]} = \int_\mathcal{R} u f_U{_{[r]}}(u) du = \int_0^1 F^{-1}(t) \frac{n!}{(r-1)!(n-r)!} t^{r-1}(1-t)^{n-p} dt
% \end{equation}
% If $U \sim \text{Uniform}[0,1]$, the expectation is equal to $EU_{[r]} = \frac{r}{n+1}$. Thus $n-r$'th order statistic from sample $n$ is on average lower than $2n-r$'th from sample $2n$, because $\frac{n-r}{n+1} < \frac{2n-r}{2n+1}$, and range between $n-r$'th and $n$'th order statistic from sample $n$ is bigger than difference between $2n-r$'th and $2n$'th order statistics from sample $2n$, since $\frac{n}{n+1} - \frac{n-r}{n+1} > \frac{2n}{2n+1} - \frac{2n-r}{2n+1}$. This simple calculation can be repeated with appropriate directions of the inequalities for the left tail of the distribution.

% For most distributions, however, this integral is intractable. Therefore, we apply approximation \cite{order_stat} $EU_{[r]} \approx F^{-1}(\frac{r}{n+1})$. For normal distribution $F^{-1}(\frac{n-r}{n+1})$ is increasing function of $n$, and  $F^{-1}(\frac{n}{n+1})- F^{-1}(\frac{n-r}{n+1})$ is decreasing with $n$. Therefore, taking greater $n$ leads to tighter tail coverage. In Figure \ref{fig:sampling}, we simulate the distribution of samples under various sampling strategies. The results indicate that reducing the sample size drawn from the buffer enhances diversity at both ends of the distribution.

\begin{figure}[htbp]
\begin{minipage}{0.95\columnwidth} % Adjust width to fit within one column
\vspace{-4mm} % Adjust vertical spacing if necessary
\begin{algorithm}[H]
\caption{Balanced Sampling}
\label{alg:modified_mir}
\begin{algorithmic}[0]
\Require Model $f$, Sample size $2C$, Task Data $D_t$, Memory $\mathcal{M}$, Parameters $\theta$
\For{$t = 1$ \textbf{to} $T$}
    \For{each $X_n$ \textbf{in} $D_t$}
        \State \textcolor{codeblue}{\%\ Would-be parameter estimate}
        \State $\theta^v \gets \text{Optimizer}(f, X_n, \theta, \alpha)$
        \State \textcolor{codeblue}{\% Select $C$ samples}
        \State $X_{C}^1 \gets \text{RandomSampling}(\mathcal{M}, C)$
        \State \textcolor{codeblue}{\% Descending sort and select top $n_1$ samples}
        \State $\{S_i^1\}_{i=1}^{n_1} \gets \text{Sort}(LossChange{}(X_{C}^1, \theta, \theta^v))$
        \State \textcolor{codeblue}{\% Select another $C$ samples}
        \State $X_{C}^2 \gets \text{RandomSampling}(\mathcal{M}, C)$
        \State \textcolor{codeblue}{\% Ascending sort and select top $n_2$ samples}
        \State $\{S_i^2\}_{i=1}^{n_2} \gets \text{Sort}(LossChange{}(X_{C}^2, \theta, \theta^v))$
        \State \textcolor{codeblue}{\% Combine the selected samples}
        \State $X_{\mathcal{M}_C} \gets \{S_i^1\}_{i=1}^{n_1} \cup \{S_i^2\}_{i=1}^{n_2}$
        \State $\theta \gets \text{Optimizer}(X_n \cup X_{\mathcal{M}_C}, \alpha)$
        \State \textcolor{codeblue}{\% Add samples to memory}
        \State $\mathcal{M} \gets \text{UpdateMemory}(X_n)$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-2mm} % Adjust if necessary
\end{figure}

The comprehensive pseudo-code for our balanced Sampling algorithm is detailed in Algorithm \ref{alg:modified_mir}.

% \subsection{Proposed Method}\label{PM}

% In this section, we integrate all components of our approach. Our algorithm selects instances from both ends of the loss chance distribution, employing a buffer-downsizing method to refine model training. This selective sampling strategy is engineered to enhance diversity within the training data, a feature especially valuable in environments with stringent memory constraints that limit data storage for training purposes. 
% The comprehensive pseudo-code for our balanced Sampling algorithm is detailed in Algorithm \ref{alg:modified_mir}.
% \vspace{-4mm}

% \begin{figure}[htbp]
% \vspace{-2mm} % Adjust vertical space as necessary
% \centering
%       \includegraphics[width=0.95\columnwidth]{figs/mir_sampling_histograms_under.png}
% \caption{Simulation of the sample distribution obtained through the implementation of different sampling strategies}
% \label{fig:sampling}
% \vspace{-2mm} % Adjust space below as necessary
% \end{figure}




==> sec/6_reviews_and_answers.tex <==
\section{Review Reply}\label{reviews}


% \section*{Review Reply}

\subsection*{General reply}

We extend our gratitude to the Reviewers for their insightful comments and suggestions regarding our work. We have addressed each Reviewer's specific questions and criticisms in their individual rebuttals.

Below, we outline the major revisions made during the rebuttal period.

\textbf{Definition of instance hardness.} We have clarified the definition of instance hardness used in our paper, including the rationale behind our choice. We differentiate our work by using logits flip instead of prediction flip. The original formula counts changes in prediction correctness, indicating a "flip" if the prediction changes from correct to incorrect or vice versa. In contrast, our metric measure the change in logits, thus capturing the magnitude of change in the model’s confidence rather than just the binary correctness of predictions.
 
\textbf{Applicability to other ER algorithms.} While our approach serves as a general plug-in for any experience replay (ER) based continual learning (CL) algorithm, we have initially combined it with the three top-performing state-of-the-art (SOTA) approaches, as other ER algorithms demonstrated inferior performance. To illustrate the ease of extending any ER method, we have added results for another popular SOTA method, DER++ (see Table 1 in the supplementary .pdf file). Due to the limited rebuttal time, results were computed for CIFAR100 and Mini-ImageNet, with remaining datasets to be completed during the discussion period and subsequently added.

\textbf{Impact of buffer size.} We concur with the Reviewers on the importance of our method's scalability concerning buffer size. Results for three different buffer sizes (1000/5000/10,000) have been added, demonstrating stable performance (see Table 2 in the supplementary .pdf file). Due to limited rebuttal time, results were computed for CIFAR100 and Mini-ImageNet, with remaining datasets to be completed during the discussion period and subsequently added.

 \textbf{Runtime.} We have included a runtime analysis of our method compared to random runtime and MIR (SOTA instance selection method). As shown in Table 3 in the supplementary .pdf file, all instance selection methods introduce runtime overhead compared to random selection. However, our approach matches the runtime of MIR while offering significantly better results.

\textbf{Online vs. class-incremental setting.} We clarified that methods such as PCR and ASER are designed for both online and traditional class-incremental settings (where one or multiple epochs can be used). To demonstrate our method's applicability in an online setting, additional experiments with a single epoch were conducted (see Table 4 in the supplementary .pdf), yielding satisfactory results. Nonetheless, our method benefits from multiple epochs, as it allows for a more accurate estimation of instance difficulty over time.
 
\textbf{Comparison with other instance selection methods.} Our initial paper included a comparison with MIR (SOTA instance selection) in the Ablation Study section. For the rebuttal, we additionally compared it with ASER, illustrating how PCR/CLSER/ERACE performs when combined with ASER versus our solution (see Table 4 in the supplementary .pdf).
 
\textbf{Hyperparameter settings.} We acknowledge the omission of important hyperparameter values in the original paper. These have now been included in Table 5 in the supplementary .pdf.
 
\textbf{Statistical significance of the results.} A Wilcoxon signed-rank test has been added to measure the statistical significance of the results. This pairwise statistical test compares two classifiers over multiple datasets. All results were obtained using 5-10 repetitions, and p-values were measured for both Accuracy and Forgetting measures, with a significance level of 0.05 (see Table 5 in the supplementary .pdf).

We hope the Reviewers find these extensions and our discussion of their comments satisfactory. We are conducting additional experiments and will share the results with the Reviewers during the Discussion Period. We look forward to further engaging with the Reviewers and discussing their comments, questions, and our responses.




\subsection*{\color{red}Reviewer 1}

\subsubsection*{Summary:}
The paper proposes a novel selection strategy for selecting which samples should be added to the rehearsal buffer memory when training a continual learning sequence of tasks. The strategy relies on promoting a reduced buffer size while sampling using both minimum and maximum interference. Furthermore, the use of this strategy is paired with an analysis of the relation between buffer size and sample diversity, and the impact on the loss function by each individual sample hardness. The first is tackled by the reduction in buffer size, while the second provides the setup for a motivational experiment that sets up the reasoning for the need of these more-varied sampling strategies.

\subsubsection*{Strengths:}
Online continual learning is an interesting topic which has most state-of-the-art methods rely on experience replay for having competitive results. Therefore, the motivation and subsequent sampling strategy would be of interest for the community of NeurIPS. The proposed strategy is simple and can be used as plug-and-play without restrictions, and therefore is easy to implement and to add to existing methods.

\subsubsection*{Weaknesses:}
Overall, the paper is a bit repetitive, taking a lot of space to provide the context as to why the proposed strategy is relevant. However, some key concepts are barely described and discussed in detail. As an example, the concept of hardness is mentioned throughout the first two pages of the submission, but the concept is only shortly explained in Figure 1 and page 3, line 136. Until then, the concept is used for motivation of the research question, but not defined or cited in any way. The main contribution is the sampling strategy, and it is compared against using it versus not using it on state-of-the-art methods. However, the sampling strategies within those methods are not discussed so much, neither is in the related work. Strategies such as herding, entropy-based sampling, or other variations of maximum interference. It would have been interesting to see the comparison on some of those methods of the strategies mentioned in Figure 3, for example. Furthermore, no statistical tests are provided over multiple runs of each method, in order to establish a better statistical significance between the use of the different sampling strategies. Instead, for the experiments provided, there is only the average of a k-fold of a single seed. Table 1 is very small and difficult to read, and Figures 4, 5, 6 would require some more clear plotting, since the color scheme provided is not intuitive to compare. Section 4.1 (datasets) could be a simple table instead. Overall, the paper seems to have limited originality, low quality of presentation of the results, requires some improvements in the writing to make some concepts more clear, and would be of some significance to the community due to the relevance of continual learning in the community. Therefore, my decision to rate the paper with a 3 (reject). However, upon further discussion with other reviewers and the answer of the questions below, I would be open to increase my rating 1 or 2 points.

\subsubsection*{Questions:}
\begin{enumerate}
    \item Is the claim that "smaller buffers promote sampling diversity" something that is only true when using the proposed strategy or something that can be extended to some other strategies?
    \item Since each task is trained for 50 epochs, how is the online continual learning setting exactly specified? How is it chosen that 50 epochs ensure thorough learning? Should each batch of data only be seen once? If you can have a short training session per task, would it be fair to compare with other rehearsal-based methods such as iCARL or IL2M? How do those methods that compensate for the recency bias affect the analysis of the sampling strategy?
    \item The definition of hardness is said to be slightly different from [50]. Which are the specific differences, and how do these provide a more intuitive evaluation of prediction-level variation?
    \item In Figure 1, could the change in level of prediction be also related to model capacity, where once enough tasks have been learned, the model starts the change between maximal and minimal interference?
\end{enumerate}

\subsubsection*{Rating:}
3: Reject: For instance, a paper with technical flaws, weak evaluation, inadequate reproducibility and/or incompletely addressed ethical considerations.

\subsubsection*{CRITIQUE:}
\begin{enumerate}
    \item No hardness definition
    \item No comparison to other sampling strategies 
    \item No statistical tests
    \item Editorial issues
    \item Smaller buffer promotes diversity- is it general claim
Class Incremental Learning vs Online learning
\end{enumerate}


\subsection*{\color{red}Reply 1}

\subsubsection*{Response to Question 1}
Smaller buffers promote sampling diversity is true in general for every selection mechanism based on statistics which is approximately normally distributed. Calculating statistics over an entire big buffer (in our case change in loss) is computationally expensive. We mitigate it by sampling a subset of a big buffer, and restricting calculations of the loss change only to sampled subset. Next we select instances from extremes for reply. Our observation is that reducing subset size promotes diversity, since k biggest values are on average more less in smaller subset. This is applicable to any selection method based on taking the extreme values of the defined statistic if its distribution is close to normal distribution.

\subsubsection*{Response to Question2} 
We are actually using class incremental learning setup but not the online learning setup. Therefore, each batch of the data is not only be visited once in each task's trainning. Therefore, when comparing with other rehearsal-based class-incremental learning methods, fair comparisons can be achieved by maintaining consistent hyperparameters. 

Recency bias in continual learning refers to the model's tendency to prioritize and remember recent experiences over older ones. Our method, however, analyzes the gradient interference of different instances. By calculating the extent to which the current gradient (from the latest batch) interferes with the gradients of past instances, our method selects instances based on their level of impact. This approach is agnostic to the age of the instance, focusing instead on the degree of interference.

\subsubsection*{Response to Question 3}
In our paper, the hardness metric is defined as the change in logits, specifically $|f_{\theta^v}(x_i) - f_{\theta}(x_i)|$, where $f_{\theta}(x_i)$ denotes the output logits for sample $i$ under model parameters $\theta$. This differs from the hardness metric presented in [50], which utilizes the concept of "prediction flip."

The "prediction flip" measures the change in a model's prediction correctness between two consecutive steps. It is defined as:

\[
\left| \mathbf{1}[\hat{y}_i^t = y_i] - \mathbf{1}[\hat{y}_i^{t-1} = y_i] \right|
\]

where $\hat{y}_i^t$ is the prediction for sample $i$ at step $t$, $y_i$ is the true label for sample $i$, and $\mathbf{1}[\cdot]$ is the indicator function that returns 1 if the condition is true and 0 otherwise.

This formula counts changes in prediction correctness, indicating a "flip" if the prediction changes from correct to incorrect or vice versa. In contrast, our metric measure the change in logits, thus capturing the magnitude of change in the model's confidence rather than just the binary correctness of predictions.

\subsubsection*{Response to Question 4}
The change in prediction levels is indeed influenced by model capacity, and as the model encounters more tasks, its output predictions naturally evolve. Our key point is that the samples with significant prediction changes differ at various stages of learning. In the early stages (the first three tasks), buffer instances with increasing loss (samples obtained through MIR) exhibit larger prediction changes. However, as the model progresses through more tasks, buffer instances with decreasing loss show larger prediction changes instead. Therefore, we argue that including both types of samples will help achieve a better balance across multiple tasks. The experimental results in the ablation study in Section 4.3 support this hybrid strategy, demonstrating improved accuracy over a single-strategy approach.


% \begin{table}[t]
% 	\centering
% 	\caption{{New Quantitative results}.}
% 	\setlength\tabcolsep{6pt}
% 	\renewcommand\arraystretch{1.1}
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{c|cc|cc|cc|cc|cc|cc}
% 			\thickhline
% 			Datasets $\&$ & \multicolumn{2}{c|}{CIFAR100}&\multicolumn{2}{c|}{Core50} &\multicolumn{2}{c|}{Food100} &\multicolumn{2}{c|}{Mini-ImageNet}&\multicolumn{2}{c|}{Places100}&\multicolumn{2}{c}{Tiny-ImageNet}\\
%                 Method & \textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )}\\
% 			\hline
%             ER\pub{ICMLW2019}\cite{chaudhry2019tiny} & 23.61 & 40.09 & 35.87 & 18.97 & 16.62 & 35.34 & 11.44 & 36.90 & 21.04 & 38.38 & 16.04 & 41.88\\ 
%             A-GEM\pub{ICLR2019}\cite{chaudhry2018efficient} & 4.10 & 75.54 & 11.22 & 63.09 & 4.14 & 67.48 & 3.92 & 74.23 & 4.47& 73.00 & 3.78 & 70.94\\
            
            
%             ASER\pub{AAAI2021}\cite{shim2021online} & 21.98 & 53.81 & 15.98 & 60.15 & 6.32 & 54.59 & 15.61 & 61.41 & 8.24 & 64.37 & 9.36 & 65.55\\
 

% \hline
%    DER++\pub{NeurIPS2020}\cite{buzzega2020dark} & 22.07 & 41.43 & 54.06 & 9.73 & 13.00 & 34.18 & 17.90 & 41.63 & 16.87 & 38.51 & 13.32 & 37.42\\
%             $+\textbf{\texttt{Ours}}$ &\reshl{\textbf{24.68}}{2.61} & \reshldown{\textbf{38.41}}{3.02} & \reshl{\textbf{TBD}}{} & \reshldown{\textbf{TBD}}{} & \reshl{\textbf{TBD}}{} & \reshldown{\textbf{TBD}}{} & \reshl{\textbf{21.62}}{3.72} & \reshldown{\textbf{40.33}}{1.30} & \reshl{\textbf{TBD}}{} & \reshldown{\textbf{TBD}}{} & \reshl{\textbf{TBD}}{} & \reshldown{\textbf{TBD}}{}\\

%                        \hline
%             ER-ACE\pub{ICLR2021}\cite{caccia2021new} & 48.85 & 14.27 & 51.36 & 12.44 & 41.81 & 17.99 & 45.53 & 15.28 & 39.55 & 25.31 & 38.95 & 17.11\\   
% 			$+\textbf{\texttt{Ours}}$ &\reshl{\textbf{50.05}}{1.20} & \reshlup{\textbf{18.31}}{4.04} & \reshl{\textbf{54.85}}{3.49} & \reshldown{\textbf{12.25}}{0.19} & \reshl{\textbf{43.13}}{1.32} & \reshlup{\textbf{18.53}}{0.54} & \reshl{\textbf{45.65}}{0.12} & \reshldown{\textbf{14.97}}{0.31} & \reshl{\textbf{40.52}}{0.97} & \reshldown{\textbf{24.41}}{0.90} & \reshl{\textbf{39.81}}{0.86} & \reshldown{\textbf{16.51}}{0.60}\\

%             \hline
%             CLS-ER\pub{ICLR2022}\cite{arani2022learning} & 48.23 & 36.24 & 47.71 & 23.56 & 45.80&34.18 & 45.60 & 36.00 & 39.71 & 40.97 & 36.28 & 40.74\\
% 			$+\textbf{\texttt{Ours}}$ &\reshl{\textbf{48.49}}{0.26} & \reshldown{\textbf{35.61}}{0.63} & \reshl{\textbf{57.74}}{10.03} & \reshldown{\textbf{17.23}}{6.33} & \reshldownred{\textbf{44.38}}{1.42} & \reshlup{\textbf{37.92}}{3.74} & \reshl{\textbf{45.87}}{0.27} & \reshldown{\textbf{35.79}}{0.21} & \reshl{\textbf{40.04}}{0.33} & \reshldown{\textbf{38.99}}{1.98} & \reshl{\textbf{37.58}}{1.30} & \reshldown{\textbf{39.28}}{1.46}\\
   
%             \hline
%             PCR\pub{CVPR2023}\cite{lin2023pcr} & 47.63 & 13.21 & 65.55 & 14.47 & 46.26 & 15.72 & 46.19 & 16.02 & 38.95 & 23.76 & 37.76 & 18.85\\
% 			$+\textbf{\texttt{Ours}}$ &\reshl{\textbf{49.96}}{2.33} & \reshldown{\textbf{12.83}}{0.38} & \reshl{\textbf{68.20}}{2.65} & \reshldown{\textbf{7.73}}{6.74} & \reshl{\textbf{48.75}}{2.49} & \reshldown{\textbf{13.17}}{2.55} & \reshl{\textbf{47.91}}{1.72} & \reshldown{\textbf{15.62}}{0.40} & \reshl{\textbf{40.69}}{1.74} & \reshldown{\textbf{20.63}}{3.13} & \reshl{\textbf{38.64}}{0.88} & \reshldown{\textbf{14.65}}{4.20}\\
% 			\hline
% 	\end{tabular}}
% 	\label{main_result}
% \vspace{-6mm}
% \end{table}



% \begin{table}[t]
% 	\centering
% 	\caption{{Results for different buffer sizes}}
% 	\setlength\tabcolsep{6pt}
% 	\renewcommand\arraystretch{1.1}
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{c|cc|cc|cc|cc|cc|cc}
% 			\thickhline
% 			Datasets & \multicolumn{6}{c|}{CIFAR100}&\multicolumn{6}{c}{Mini-imagenet}\\
%             \hline
%             Buffer Size & \multicolumn{2}{c|}{1000} & \multicolumn{2}{c|}{5000} & \multicolumn{2}{c|}{10000} & \multicolumn{2}{c|}{1000} & \multicolumn{2}{c|}{5000} & \multicolumn{2}{c}{10000}\\
%             \hline
%             Methods & \textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )} &\textit{Acc. ($\uparrow$ )} &\textit{Fgt. ($\downarrow$ )}\\
%             \hline
%             ER-ACE\pub{ICLR2021} & 30.35 & 37.99 & 43.07 & 18.72 & 48.85 & 14.27 & 36.96 & 27.70 & 40.05 & 21.46 & 45.53 & 15.28\\   
%             $+\textbf{\texttt{Ours}}$ &\reshl{\textbf{30.54}}{0.19} & \reshldown{\textbf{34.50}}{3.49} & \reshl{\textbf{44.40}}{1.33} & \reshlup{\textbf{24.17}}{5.45} & \reshl{\textbf{50.05}}{1.20} & \reshlup{\textbf{18.31}}{4.04} & \reshl{\textbf{TBD}}{0.00} & \reshldown{\textbf{TBD}}{0.00} & \reshl{\textbf{TBD}}{0.00} & \reshldown{\textbf{TBD}}{0.00} & \reshl{\textbf{45.65}}{0.12} & \reshldown{\textbf{14.97}}{0.31}\\
%             CLS-ER\pub{ICLR2022} & 21.70 & 65.81 & 42.06 & 42.92 & 48.23 & 36.24 & 18.21 & 67.72 & 39.01 & 44.10 & 45.60 & 36.00\\
%             $+\textbf{\texttt{Ours}}$ &\reshl{\textbf{22.23}}{0.53} & \reshldown{\textbf{65.53}}{0.28} & \reshl{\textbf{42.16}}{0.10} & \reshldown{\textbf{42.13}}{0.79} & \reshl{\textbf{48.49}}{0.26} & \reshldown{\textbf{35.61}}{0.63} & \reshldownred{\textbf{17.88}}{0.33} & \reshlup{\textbf{68.17}}{0.95} & \reshl{\textbf{39.82}}{0.81} & \reshlup{\textbf{44.11}}{0.01} & \reshl{\textbf{45.87}}{0.27} & \reshldown{\textbf{35.79}}{0.21}\\
%             PCR\pub{CVPR2023}\cite{lin2023pcr} & 29.24 & 24.66 & 43.31 & 16.18 & 47.63 & 13.21 & 24.37 & 42.63 & 40.86 & 21.66 & 46.19 & 16.02\\
%             $+\textbf{\texttt{Ours}}$ &\reshl{\textbf{30.80}}{1.56} & \reshldown{\textbf{22.38}}{2.28} & \reshl{\textbf{45.14}}{1.83} & \reshldown{\textbf{16.12}}{0.06} & \reshl{\textbf{49.96}}{2.33} & \reshldown{\textbf{12.83}}{0.38} & \reshl{\textbf{26.94}}{2.57} & \reshldown{\textbf{38.67}}{3.96} & \reshl{\textbf{42.54}}{1.68} & \reshldown{\textbf{20.01}}{1.65} & \reshl{\textbf{47.91}}{1.72} & \reshldown{\textbf{15.62}}{0.40}\\
% 			\hline
% 	\end{tabular}}
% 	\label{main_result}
% \vspace{-6mm}
% \end{table}




\begin{table}[h!]
\centering
\caption{Comparison of running times per epoch on different datasets using PCR as backbone.}
\begin{tabular}{|l|c|c|c|}
\hline
PCR & random & MIR & OURS \\ \hline
mini-imagenet & 16s & 36s & 36s \\ \hline
cifar100 & 8s & 29s & 29s \\ \hline
\end{tabular}

\label{table:pcr_comparison}
\end{table}

\begin{table}[h!]
\centering
\caption{Comparison of different online settings across CIFAR100 and Mini-imagnet datasets.}
\begin{tabularx}{\textwidth}{|l|X|X|X|X|X|X|}
\hline
 \scriptsize Online Accuracy& \scriptsize \textbf{PCR+ASER} & \scriptsize \textbf{PCR+OURS} & \scriptsize \textbf{CLSER+ASER} & \scriptsize \textbf{CLSER+OURS} & \scriptsize \textbf{ERACE+ASER} & \scriptsize \textbf{ERACE+OURS} \\ \hline
\textbf{CIFAR100} & 28.42 & 29.03 & 13.03 & 10.89 & 15.26 & 15.89 \\ \hline
\textbf{Mini-imagnet} & 26.63 & 27.97 & 12.71 & 12.04 & 12.47 & 11.62 \\ \hline
\end{tabularx}

\label{table:online_settings_swapped}
\end{table}



\begin{table}[h!]
\centering
\caption{Results of Wilcoxon signed-rank test for comparison over mutiple datasets with significance level = 0.05}
\begin{tabular}{|l|c|c|}
\hline
 & Acc. ($p$-values) & Fgt. ($p$-values) \\ \hline
ER-ACE+Ours vs. ER-ACE & 0.0000 & 0.0177 \\ \hline
 CLS-ER+Ours vs. CLS-ER & 0.0068 & 0.0082 \\ \hline
PCR+Ours vs. PCR & 0.0000  & 0.0000 \\ \hline
\end{tabular}
\end{table}
% \begin{table}[h!]
% \centering
% \caption{Hyperparameter Settings}
% \label{tab:hyperparameters}
% \renewcommand{\arraystretch}{1.1} % Adjust this value to change the row spacing
% \begin{tabular}{>{\raggedright\arraybackslash\footnotesize}m{3cm} | >{\raggedright\arraybackslash}m{3.5cm} |>{\raggedright\arraybackslash\footnotesize}m{3.5cm} | >{\raggedright\arraybackslash}m{3cm}}
% \toprule
% \textbf{Hyperparameter} & \textbf{Value} & \textbf{Hyperparameter} & \textbf{Value} \\
% \midrule
% Optimizer & SGD & Weight Decay & 0 \\
% Learning Rate & 0.1 & Epoch & 50 \\
% Training Batch Size & 10 & Testing Batch Size & 128 \\
% Number of Tasks & 20 & Instances Retrieved Per Batch & 10 \\
% Weight Initialization & Xavier Uniform & CLSER Consistency Regularization Weight & 0.1 \\
% CLSER Stable Model Update Freq & 0.7 & CLSER Stable Model Alpha & 0.999 \\
% CLSER Plastic Model Update Freq & 0.9 & CLSER Plastic Model Alpha & 0.999 \\
% DER++ Alpha & 0.5 & DER++ Beta & 0.5 \\
% \bottomrule
% \end{tabular}
% \end{table}


\subsection*{\color{red}Reviewer 2}

\subsubsection*{Weaknesses:}
\begin{itemize}
    \item \textbf{Risk of Overfitting:} The approach favors smaller memory buffers to increase diversity, but there's insufficient discussion on the potential risk of overfitting or increased volatility in learning due to the reduced number of instances available for replay.
    \item \textbf{Computational Cost:} There is a lack of discussion on the computational implications of the proposed method. While the paper claims the method is a "simple and low-cost plugin," there is no substantial analysis of runtime or computational costs.
    \item \textbf{Lack of different buffer sizes:} The omission of buffer sizes in Table 1 is a significant oversight, complicating the assessment of the method’s scalability or adaptability under different memory constraints. Additionally, the extremely low accuracy reported for A-GEM across multiple datasets raises questions about either the implementation or the appropriateness of the comparison setup.
    \item \textbf{Limited Testing Scope:} The paper claims the proposed method can serve as a plugin for any experience replay method, yet it only demonstrates integration with three specific methods (as shown in Table 1). This limited scope restricts evidence of its general applicability. Demonstrating the method's effectiveness across a broader range of experience replay methods could better substantiate its versatility and general utility.
    \item \textbf{Insufficient Comparison:} More detailed comparisons with alternative instance selection strategies could strengthen the paper's claims. The paper does not sufficiently differentiate its methodology from existing approaches like those referenced in the paper. (The related work section does not comprehensively cover the existing literature, particularly recent advancements in continual learning that are directly relevant to the paper’s topic. This oversight raises concerns about whether the proposed method sufficiently advances beyond the current state of the art.) The proposed approach, which involves selecting instances from both extremes of the loss distribution, appears to be an incremental variation on existing memory replay strategies. The methodology section, while detailed, lacks a robust theoretical framework that sets it apart from existing methods. The discussion lacks a critical analysis of why certain datasets show only marginal improvements and does not address potential limitations or failures of the proposed strategy.
    \item \textbf{Organizational Issues:} The paper is generally well-written but suffers from several organizational issues. Some sections are overly verbose, particularly in the literature review, which could be streamlined to focus more on gaps that the current work aims to fill. There is a disconnect between the methods tested and the conditions under which they were intended to operate. Specifically, ASER and PCR, which are designed for online continual learning, are inappropriately tested in an offline setup with multiple epochs (50 epochs instead of 1). The paper does not mention if the results were averaged over multiple runs, which is a standard practice to ensure the reliability and generalizability of the findings. This omission casts doubt on the statistical robustness of the reported improvements.
    \item \textbf{Lack of Hyperparameter Details:} The paper fails to clearly specify hyperparameters used in the experiments, referencing configurations from the Mammoth framework without providing direct details for replication. The lack of available hyperparameter details of dataset CIFAR100, and Core50 for CLS\_ER in its official repository and paper further complicates the ability to reproduce and verify the results, challenging the paper’s claims about following established configurations.
    \item \textbf{Influence on Decision Boundaries:} While the paper effectively addresses instance hardness and buffer diversity, it lacks a thorough exploration of how these factors influence the decision boundaries of the models. This is critical for understanding the full implications of the instance selection strategy on model performance.
\end{itemize}

\subsubsection*{Questions:}
see weaknesses
\subsubsection*{CRITIQUE:}
\begin{enumerate}
    \item Overfitting
    \item Computational cost 
    \item Different buffer sizes
    \item Only three ER methods
    \item Related works not sufficient
    \item Where method does not work
    \item Lack of experimental details, hyperparameters results presentation/statistical significance 
    
\end{enumerate}


\subsection*{\color{red}Reply 2}

\textbf{Risk of Overfitting:} The main way of measuring the overfitting of the model is analyzing its generalization capabilities. The experimental results provided by us show that our method, despite using a small buffer, leads to improved classification performance and reduced forgetting (and thus robustness to overfitting). We show that the size of the buffer is secondary to its composition and that using diverse instances in it leads to improvements in generalization. This is in line with the SOTA understanding of the overfitting phenomena, which often stems from not capturing all representative concepts in data or overtraining on non-diverse information. We will add discussion to the paper. 

\textbf{Computational Cost:} Our claims on our method being a simple and low-cost plugin were coming mainly from the fact that we focused on understanding the actual mechanism behind the interplay among instance selection, instance difficulty, and CL; rather than proposing an overly complicated mechanism. Our focus was on showing that asking the right question “what do we need for ER to work” is more important than coming up blindly with more and more replay strategies. Our method has identical computational complexity as other retrieval methods such as MIR, which of course always adds extra runtime when compared with random selection. However, as shown in ablation study, we offer a superior performance to MIR (with same runtime, see Table 3 in supplementary .pdf)

 \textbf{Lack of different buffer sizes:} We have added an analysis of different buffer sizes [1000/5000/10000] (see Table 2 in supplementary .pdf). We can see that our diverse instance selection leads to improved results for all three examined buffer sizes, proving its scalability and capability to work under different resource constraints. As for A-GEM, we are using popular and publicly vetted implementation from https://github.com/RaptorMai/online-continual-learning. Furthermore, multiple recent papers report almost identical, extremely low performance of A-GEM when dealing with a high number of tasks / classes (see e.g., PCR: Proxy-Based Contrastive Replay for Online Class-Incremental Continual Learning [CVPR23] or Retrospective Adversarial Replay for Continual Learning [NeurIPS22]). We are certain that A-GEM results are correct.
 
\textbf{Limited Testing Scope:} We have selected three SOTA ER (ICLR21/ICLR22/CVPR23) to be combined with our approach. The remaining reference methods performed significantly worse than these three, so we focused on SOTA. We have added a comparison with another SOTA DER++ [NeurIPS20] (see Table 1 in supplementary .pdf) that also shows favorable improvements offered by our diverse instance selection. Due to the short time for rebuttal, we can present only results for DER++ and 2 datasets – remaining results will be added during the discussion period. 

 \textbf{Insufficient Comparison:} In our paper, we have showed a comparison between our method and Maximally Interfered Retrieval (MIR, [NeurIPS19]), which is considered one of the best instance selection strategies for CL. We have now added a comparison between our selection strategy and another instance selection SOTA: Adversarial Shapley Value Experience Replay (ASER, [AAAI21]). Please refer to Table 4 in supplementary .pdf added to the Author rebuttal for comparison between ASER and our method, both used as plugins to PCR/CLSER/ERACE and showcasing that our method leads to better performance improvements for all three ER. 
 
 \textbf{Organizational Issues:}  We appreciate the suggestions on rewriting the related works section and will follow accordingly. However, we must politely disagree with the comment on the lack of insights into how our method differs from SOTA in memory retrieval for ER. We have pointed out the need for analyzing the instance difficulty in CL and showed that selecting only the most difficult instances (or more broadly – extreme values according to any selection criterion) leads to a lack of diversity in the composed buffer. We have followed this with a theoretical analysis of the impact of the buffer size on the diversity of the buffer, showing that we need to rethink how instances are being chosen during the instance selection process. While the improvements may differ among 6 used datasets (which is to be expected when using more datasets), we can see that in most cases adding our selection method helps improve generalization and reduce forgetting.
 
\textbf{Testing conditions:} All the presented results were averaged over 5-10 runs (see sec 4.2 in the paper, we incorrectly called it folds). We have added statistical tests of significance for pairwise comparison between PCR/CLSER/ERACE without any instance selection, with ASER, and with our method, showing that our approach offers statistically significant improvements. (see Table 6 in supplementary .pdf).

\textbf{Lack of Hyperparameter Details:} We have added details of the used hyperparameters to facilitate the reproducibility of our study (see Table 5 in supplementary .pdf)

\textbf{Influence on Decision Boundaries:} Our  work focuses on exploiting the instance hardness in CL, showing that exploring relaxed extrema in instance selection leads to better generalization and reduced forgetting. While we haven’t explicitly addressed the impact on decision boundaries, this is a very important aspect of instance selection. As discussed with the paper, we have noticed that there are a lot of instances in the buffer that maintain the high ratio of logits flip even when loss is decreasing. This is most likely selecting instances on the decision boundaries, allowing our method to better focus on preserving the boundaries of old tasks, while incorporating new knowledge. Thus, by exploring the impact of instance difficulty on CL, we are implicitly analyzing the impact on decision boundaries. 



\subsection*{\color{red}Reviewer 3}



\subsubsection*{Weaknesses:}
In several parts of the document, the way the paper is written makes it difficult to understand the definition of some concepts. For example:
\begin{itemize}
    \item One such instance is the authors' use of the term 'buffer size'. In the contributions and summary, they discuss reducing the buffer size, a concept typically associated with the size of samples saved from previous distributions in most previous work. However, their approach seems to focus more on reducing the element sample to form the buffer, which can lead to confusion for readers.
    \item \textbf{Online Learning versus CIL:} The authors discuss performing experiments in a Class Incremental Learning setup in the problem formulation and the experiments section. However, their experimental setup is extracted and is similar to an online approach, with the main difference being that they perform 50 epochs of training per task. So, they assume some hyper-parameters (like the batch size) for an online approach but train for 50 epochs (like a CIL), creating confusion in selecting the hyper-parameters.
    \item \textbf{Lack of Experiments on Buffer Size:} One of the authors' motivations is to reduce the buffer size. However, a significant gap is the lack of experiments demonstrating how performance changes when the buffer (or batch) size is altered. The authors' hypotheses, as they acknowledge in the paper, are some of them counterintuitive, but without empirical results, these hypotheses remain unproven.
    \item \textbf{Efficiency Concerns:} One of the motivations for the new method is efficiency. Again, showing experiments is necessary to prove that this contribution is fulfilled. Also, probing this motivation is more complex if we analyze that the proposed algorithm does a double optimization process for each batch, as described in Algorithm 1.
    \item \textbf{Figure Readability:} Figs. 1, 2, and 3 have very small labels. The authors should consider increasing the font size of the figures.
    \item \textbf{Figure Legend Matching:} The figures' colours have to match the legend's. Ideally, the legend should be added to the figure.
    \item \textbf{Writing Quality:} The list of numbers on lines 315-317 shows a lack of time to write the paper properly. To improve the presentation, it can be transformed into a figure that can go into the Appendix.
\end{itemize}

\subsubsection*{Questions:}
\begin{enumerate}
    \item What memory size is used in the experiments? Does the memory size affect the current conclusions? For example, a larger memory size may include a larger number (and more diverse) of samples but decrease the variability since most can reflect only the most popular part of the distribution.
    \item Studying how the results change when modifying the memory size might be interesting.
    \item The authors talk about sampling only a small number of data, but why? Did you do experiments sampling more data per batch?
    \item On the other hand, several papers discuss what elements to add to memory (Storage Policy). How does this affect your proposal? Some papers talk about adding more diversity to the memory, which may be similar to the proposed idea. Can you discuss the difference between the two approaches? 
    \begin{itemize}
        \item Rebuffi, Sylvestre-Alvise, et al. "iCaRL: Incremental classifier and representation learning." Proceedings of the IEEE conference on Computer Vision and Pattern Recognition. 2017.
        \item Hayes, Tyler L., and Christopher Kanan. "Selective replay enhances learning in online continual analogical reasoning." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2021.
        \item Hurtado, Julio, et al. "Memory Population in Continual Learning via Outlier Elimination." Proceedings of the IEEE/CVF International Conference on Computer Vision. 2023.
    \end{itemize}
    \item The analysis carried out in section 3.2 is based on an Online Learning approach. Have you explored the hyper-parameters for a CIL environment? This change can significantly impact the insights and results obtained.
    \item Which hyper-parameters were used for the other methods? Were they the same ones mentioned in the setup section, or were the ones shown in each original paper? Was a search for hyper-parameters carried out?
    \item Why use such a small batch? This decision makes sense in online learning scenarios but not so much in CIL.
    \item In line 136, you mention using a slightly different hardness metric. Could you explain the rationale behind this and how it affects the final results? I appreciate the thought that went into this decision.
    \item Section 3.3 discusses increasing the diversity of samples when reducing the sample size drawn from the buffer. But if we go to the extreme, the most diverse batch is the one that is sampled over the entire buffer. Intuitively speaking, what are the advantages of sampling over extremes?
    \item In Table 1, what would the results be when sampling only the tops without random sampling first?
    \item Could you clarify the difference between random sampling and then selection, selecting the K (where K >> n) top samples and then random sampling from them? Your insights on this could help me better understand the methodology.
    \item Methods based on pre-trained models are gaining much ground. Can this method also benefit approaches based on these models?
\end{enumerate}

\subsubsection*{CRITIQUE:}
\begin{enumerate}
    \item Class Incremental Learning vs Online learning
    \item Buffer size vs subbuffer size
    \item Different buffer sizes
    \item Hyperparameters
    \item Related works not sufficient
    \item Hardness definition
    \item Diversity is biggest while sampling from entire buffer
    \item Usage with pretrained models 
    
\end{enumerate}

\subsection*{\color{red}Reply 3}
\begin{enumerate}
    \item (For question 1 and 2)In Table 1, the quantitative results for six different datasets were obtained with a buffer size of 10,000. However, our method achieves comparable results using only half the buffer size, 5,000. Additionally, Table 2 presents results for three different buffer sizes[1000/5000/10000] on CIFAR-100 and Mini-ImageNet, further validating that our conclusions remain consistent across varying buffer capacities.
    \item For each batch, we sample an equal number of instances corresponding to the batch size, applying this approach uniformly across all comparison methods to ensure fairness. We do not conduct experiments involving sampling more data per batch.
    \item The iCarl method constructs sets of prototypes for each class and employs a nearest-mean-of-exemplars strategy for classification. In contrast, our method uses experience replay to mitigate catastrophic forgetting. Samples are selected for the large memory buffer regardless of their labels and are then added to batches of new data to prevent forgetting. Our research focuses on the question: which samples from the large memory buffer should be added to the current data batch?

    The paper "Selective Replay Enhances Learning in Online Continual Analogical Reasoning" evaluates different selective replay methods across various datasets, comparing selection mechanisms based on statistics such as minimum confidence and maximum margin. Samples with the highest or lowest values of a particular statistic are chosen from the large memory buffer. Our work complements this approach by arguing for selecting samples from both extremes of these statistics and reducing the size of the subset from which we draw samples. We perform experiments based on loss change statistics.
    
    The paper "Memory Population in Continual Learning via Outlier Elimination" eliminates outliers from the buffer and samples it uniformly. Our method selects samples based on the loss change statistic. Incorporating buffer cleaning into our method before drawing a subset, calculating loss change, and selecting instances to replay could be an interesting direction for future research.

    \item The analysis in Section 3.2 is based on instance-level evaluation of PCR, using a random buffer retrieval and update strategy. This involves dividing CIFAR-100 into 20 tasks and training each task for 50 epochs in a class-incremental setup. According to its authors, PCR is designed as an online class-incremental learning framework, and experiments have demonstrated its effectiveness for both online learning and class-incremental learning.

    \item The hyperparameters that we used are shown in table 4, only DER++ and CLSER have unique hyperparameters not present in other models. For these hyperparameters, we used the default value from the original implementation.

    \item Research has shown that in continual learning scenarios, smaller batch sizes can lead to better accuracies:
    \begin{enumerate}
        \item Understanding the Role of Training Regimes in Continual Learning.[NeurIPS 2020]
        \item Remember More by Recalling Less: Investigating the Role of Batch Size in Continual Learning with Experience Replay. [AAAI 2021]
    \end{enumerate}
    Both of these papers point out to an excellent performance of batch size 10 in continual learning. Additionally, we aim to maintain consistency in hyperparameters across different datasets, including those with larger image sizes.

    \item In our paper, the hardness metric is defined as the change in logits, specifically $|f_{\theta^v}(x_i) - f_{\theta}(x_i)|$, where $f_{\theta}(x_i)$ denotes the output logits for sample $i$ under model parameters $\theta$. This differs from the hardness metric presented in "Curriculum learning by dynamic instance hardness. [NeurIPS 2020]", which utilizes the concept of "prediction flip."

    The "prediction flip" measures the change in a model's prediction correctness between two consecutive steps. It is defined as:
    
    \[
    \left| \mathbf{1}[\hat{y}_i^t = y_i] - \mathbf{1}[\hat{y}_i^{t-1} = y_i] \right|
    \]
    
    where $\hat{y}_i^t$ is the prediction for sample $i$ at step $t$, $y_i$ is the true label for sample $i$, and $\mathbf{1}[\cdot]$ is the indicator function that returns 1 if the condition is true and 0 otherwise.
    
    This formula counts changes in prediction correctness, indicating a "flip" if the prediction changes from correct to incorrect or vice versa. In contrast, our metric measure the change in logits, thus capturing the magnitude of change in the model's confidence rather than just the binary correctness of predictions.
    
    \item (For question 9, 10 and 11)Sampling only tops from the big buffer is very costly since it requires the calculation of the change of loss for the entire buffer. Random sampling decreases the sample size from which samples with the highest loss change are chosen. Assume we choose $n$ samples from a buffer with size $k$. Then the sample with the lowest loss change from $n$ samples with the highest loss change chosen from the whole buffer approximates $\frac{k-n}{k + n}$-th percentile. Decreasing $k$, on average, promotes less extreme values of the loss change.

    \item In continual learning, the primary goal is to enable a model to learn incrementally from a stream of data without forgetting previously learned information. Using pre-trained weights, as in transfer learning, typically involves pre-training on a large dataset and fine-tuning on a smaller target dataset, which can make the model heavily reliant on the initial pre-trained weights. While this approach may be an interesting direction, this paper focuses on selecting more influential instances from the buffer.

    
\end{enumerate}
\subsection*{\color{red}Reviewer 4}

\subsubsection*{Weaknesses}
Detail in Methodology: Some parts of the methodology, particularly the mathematical formulations, could benefit from more detailed explanations to enhance understanding for readers who may not be deeply familiar with the technical specifics.

Visual Aids: The inclusion of more visual aids, such as diagrams and flowcharts, could help clarify complex concepts and improve the overall presentation.

Broader Evaluation: While the paper evaluates the method on several datasets, additional experiments on a more diverse range of tasks could further validate the generalizability of the proposed approach. For example, different orders of sequentially emerged tasks across different datasets.

\subsubsection*{Questions}
\begin{enumerate}
    \item Can the authors provide more detailed explanations or examples of how the proposed hardness metric is calculated and applied in different scenarios?
    \item Are there any specific limitations in the computational resources required for implementing the proposed method, especially in large-scale applications?
    \item How does the method perform when integrated with other continual learning strategies beyond those mentioned in the paper?
    \item Can the authors provide insights into potential real-world applications where this method could be particularly beneficial?
\end{enumerate}


\subsubsection*{CRITIQUE:}
\begin{enumerate}
    \item More detailed mathematical formulation of methodology
    \item Broader evaluation
    \item Hardness definition
    \item Memory requirements
    \item Other ER
    \item Practical usage 
    
\end{enumerate}

\subsection*{\color{red}Reply 4}

\begin{enumerate}
    \item In our paper, we define the hardness metric as the change in logits, specifically \( |f_{\theta^v}(x_i) - f_{\theta}(x_i)| \), where \( f_{\theta}(x_i) \) represents the output logits for sample \( i \) under model parameters \( \theta \). This is in contrast to the hardness metric introduced in "Curriculum Learning by Dynamic Instance Hardness" (NeurIPS 2020), which employs the concept of "prediction flip."

    The "prediction flip" metric measures the change in a model's prediction correctness between two consecutive steps. It is defined as:
    
    \[
    \left| \mathbf{1}[\hat{y}_i^t = y_i] - \mathbf{1}[\hat{y}_i^{t-1} = y_i] \right|
    \]
    
    where \( \hat{y}_i^t \) denotes the prediction for sample \( i \) at step \( t \), \( y_i \) is the true label for sample \( i \), and \( \mathbf{1}[\cdot] \) is the indicator function that returns 1 if the condition is true and 0 otherwise.
    
    This formula accounts for changes in prediction correctness, indicating a "flip" if the prediction changes from correct to incorrect or vice versa. In contrast, our metric measures the change in logits, thereby capturing the magnitude of change in the model's confidence, rather than solely the binary correctness of predictions.

    \item Our method improves the performance of all three state-of-the-art (SOTA) methods across six datasets with diverse image sizes. Additionally, for large-scale applications, users can flexibly adjust the batch size based on data volume and device storage capacity, ensuring optimal efficiency and resource utilization. 

    \item Our method is straightforward and can be seamlessly integrated into existing systems as a plug-and-play solution, making it easy to implement without any restrictions. Our experiments have demonstrated its effectiveness with three state-of-the-art methods. Additionally, it is a valuable option to consider for any continual learning method that utilizes a memory buffer.

    \item Our methods are ideal for scenarios with ample storage and a continuous influx of new data, where retraining costs are prohibitive. Such scenarios include models used in social media analytics, financial stock market predictions, etc..
    

\end{enumerate}
